Constant delay algorithms for regular document spanners

Regular expressions and automata models with capture variables are core tools in rule-based information extraction. These formalisms, also called regular document spanners, use regular languages in order to locate the data that a user wants to extract from a text document, and then store this data into variables. Since document spanners can easily generate large outputs, it is important to have good evaluation algorithms that can generate the extracted data in a quick succession, and with relatively little precomputation time. Towards this goal, we present a practical evaluation algorithm that allows constant delay enumeration of a spanner's output after a precomputation phase that is linear in the document. While the algorithm assumes that the spanner is specified in a syntactic variant of variable set automata, we also study how it can be applied when the spanner is specified by general variable set automata, regex formulas, or spanner algebras. Finally, we study the related problem of counting the number of outputs of a document spanner, providing a fine grained analysis of the classes of document spanners that support efficient enumeration of their results.

==> constantdelayversion.tex <==
Assume that \texttt{stack} is a global stack with the standard stack methods  \texttt{push} and \texttt{pop}. Furthermore, assume that the list data structure is realized by adding the \texttt{next} component to the node data structure as well. That is, we have a \texttt{next()} method for a list that will return the next node in the list, as before. This iterator will be implemented by allowing each node to be linked to the next node on the list using the component \texttt{next}. If the node $n$ is not connected to another node, we assume that $n.\texttt{next}=\texttt{null}$. Note that by Algorithm \ref{alg:ma-eval} we never link a node to two different nodes.

The constant delay version of Algorithm \ref{alg:output} is given in Algorithm \ref{alg:output1}. The main idea here is to use a stack in order to keep track of when there is a branch in the directed acyclic graph that stores all the runs, and, instead of backtracking step by step to this point, jumping to it directly in order to produce an output. This allows us to produce each output in time that is linear in the output's length, and take constant time between two different outputs. 

\begin{algorithm}
	\caption{Enumerate all mappings in constant delay}\label{alg:output1}
	\begin{algorithmic}[1]
		\Procedure{{Enumerate}}{$\{\plist_q\}_{q \in Q}$, $F$}
		\ForAll{$q \in F$ \textbf{with} $\plist_q \neq \epsilon$}
		\State {\tt stack.init()}
		\State $\textsc{Enum}(\plist_q,\epsilon)$
		\EndFor
		\EndProcedure
		
		\smallskip
		
		\Procedure{{Enum}}{$\plist, \newmap$}
		
		\State $\plist\!.{\tt begin}$
		
		\If{$\plist\!.{\tt atEnd} = {\tt false}$}
			\State $\newnode \gets \plist\!.{\tt next}$
			\If{$\newnode \neq \bot$}
				\State $(S, i) \gets \newnode.{\tt content}$
				\State $\texttt{nxt} \gets \newnode.{\tt next}$
				\If{$\texttt{nxt} \neq \texttt{null}$}		
					\State $\texttt{stack.push((nxt,map))}$
				\EndIf
				\State $\textsc{Enum}(\newnode.{\tt list}, \,(S, i) \cdot \newmap)$		
			\Else
				\State ${\tt Output}(\newmap)$
				\State $\texttt{nxt} \gets \texttt{stack.pop()}$
				\If{$\texttt{nxt}\neq \texttt{null}$}
					\State $(S, i) \gets \texttt{nxt.node.content}$
					\State $\newmap \gets \texttt{nxt.map}$
					\State $\texttt{newnxt} \gets \texttt{nxt.node.next}$
					\If{$\texttt{newnxt}\neq \texttt{null}$}
						\State $\texttt{stack.push((newnxt,map))}$
					\EndIf
					\State $\textsc{Enum}(\texttt{nxt.node.list}, \,(S, i) \cdot \newmap)$		
				\EndIf
			\EndIf
		
%		\While{$\plist\!.{\tt atEnd} = {\tt false}$}
%				\State $\newnode \gets \plist\!.{\tt next}$
%				
%				\If{$\newnode = \bot$}
%					\State ${\tt Output}(\newmap)$
%				\Else
%					\State $(S, i) \gets \newnode.{\tt content}$
%					\State $\textsc{Enum}(\newnode.{\tt list}, \,(S, i) \cdot \newmap)$
%				\EndIf			
%		\EndWhile
		\EndIf
		\EndProcedure
	\end{algorithmic}
\end{algorithm}

==> join.tex <==



==> seq_ext.tex <==
We first prove that for any sequential $\VA$ $\cA$ there exists an equivalent $\dsEVA$ $\cA'$ with at most $2^n$ states and $2^n(2^\ell n^2+|\Sigma|)$ transitions. 
As showed in the previous proof, there exists a family of sequential automatons with an exponential blow-up in the number of possible transitions for any equivalent $\EVA$. This blow-up follows from the fact that for every two states $q$ and $q'$ in $\cA$, all paths between them just have the same markers that are only open or only close. Formally, for a variable path $\pi$ in $\cA$ (see the definition of variable path in the Proof of Theorem \ref{theo:equivalence}), let $T_\pi \subseteq \markers(\pi)$ be the set of variables $v$ such that either $\Open{v} \in  \markers(\pi)$ or $\Close{v} \in \markers(\pi)$, but not both.
\begin{lemma}
	If $\cA$ is sequential, then for every two states $q$ and $q'$ in $\cA$ that can produce valid runs, it holds that $T_{\pi} = T_{\pi'}$ for every variable paths $\pi$ and $\pi'$ between $q$ and $q'$.
\end{lemma}

	
\begin{proof}
	  If the property does not hold, then there are two states $q$ and $q'$ in $\cA$ and two variable paths $\pi$ and $\pi'$ between $q$ and $q'$ such that $T_\pi \neq T_{\pi'}$. Without lost of generality, assume that $\Open{x} \in T_\pi$ but $\Open{x} \notin T_{\pi'}$ (the other cases are similar). Since $q$ and $q'$ can produce valid runs, then they are both reachable from $q_0$ and can reach a final state. Specifically, let $\pi_i$ be the path from $q_0$ to $q$, and $\pi_f$ be the path from $q'$ to a final state. Given that $\Open{x} \in T_\pi$, then $\Close{x}$ must appear once in $\pi_f$, since the concatenated run $\pi_i \pi \pi_f$  is valid. Yet, $\cA$ is sequential, therefore $\pi_i \pi' \pi_f$ should also be valid.
	 This leads to a contradiction since $\pi_i \pi' \pi_f$  only closes $x$ and never opens it, which implies that  $\pi_i \pi' \pi_f$ is not valid.
	 %The other case is similar, if $\Close{x}$ appears in $\pi$, then $\Open{x}$ appears once in the path $\pi_i$. Again, since $\cA$ is sequential, $\pi_i \pi' \pi_f$ should also be valid, but is only opens $x$ and never closes it. Both possibilities arrive to a contradiction. 
	 Therefore the property holds. 
\end{proof}

The previous lemma shows that different variable paths $\pi$ between states can differ only in the complement of $T_{\pi}$, namely, all variables such that they both open and close in the path. Indeed this is true, since if all paths have different opened and closed variables, valid runs can still be established, they will not define mapping in the same variables, but are valid nonetheless. Therefore, a path may have any subset of the variables, as long both the opening and closing marker appear in them. So, in the worst case, $2^\ell$ extended marker transitions may be established between two states. Therefore, if $\cA_{\text{ext}}$ is the $\EVA$ resulting of our construction, such that $\cA\equiv \cA_{\text{ext}}$, then it has at most $m + 2^\ell\cdot n^2$ transitions. If we add the fact that equivalent $\dsEVA$ $\cA'$ can be constructed (Proposition \ref{prop:determinization}), then $\cA'$ has at most $2^n$ states and $2^n (2^\ell n^2 + |\Sigma|)$ transitions.

%The proved property for every path between two states $q$ and $q'$ in $\cA$, considered any kind of path, yet, we showed our construction considers adding transitions only where variable-paths exists, as the ones that only contain marker transitions. Then, the resulting bound for transitions also follows if we consider the property for this kind of transitions. 
Now, if we consider $\epsilon$-free sequential $\EVA$ $\cA$, then any variable-path in $\cA$ cannot contain both opening and closing marks for a single variable. Otherwise, following that path on an accepting run would produce a $\epsilon$ mapping for a variable.
Thus, all variable paths between two states may only contain the same set of markers (only opening or closing for each variable), and at most one extended marker transition could be added, per pair of states. This brings back the bound to $2^n(n^2+|\Sigma|)$ transitions for $\epsilon$-free sequential $\EVA$.

==> spanners.tex <==
%!TEX root = ../main/main.tex

The previous section shows an algorithm that evaluates a deterministic
sequential extended VA (\dsEVA) $\cA$ over a document $d$ with
constant-delay enumeration after $O(|\cA|\times |d|)$
preprocessing. However, the wider objective of this algorithm is to
evaluate regular spanners. In this section, we present a fine-grained
study of the complexity of transforming an arbitrary regular spanner,
expressed in any of $\RGX$, $\VA$, $\RGX^{\{\pi,\cup,\Join\}}$ or
$\VA^{\{\pi,\cup,\Join\}}$ to a $\dsEVA$. This hence identifies  the
cost of the  algorithm of Section~\ref{sec:algorithm} for evaluating
regular spanners.

It is well-known that $\RGX$ formulas can be translated into $\VA$ in
linear time~\cite{FKRV15}. Therefore, we focus our study on the
setting where spanners are expressed in $\VA^\algops$. We first
study how to translate arbitrary $\VA$s into $\dsEVA$s, and then turn to the
algebraic constructs.  For the sake of simplification, in this section
we assume the following notation: for any VA $\cA = (Q, q_0, F,
\delta)$, $n = |Q|$ denotes the number of states, $m = |\delta|$ the
number of transitions, and $\ell = |\var(\cA)|$ the number of
variables in $\cA$.

From a $\VA$ we can obtain a sequential $\VA$ by using a construction similar to the one presented in~\cite{F17}. This yields an automaton with $2^n3^\ell$ states. This sequential VA can be then extended and determinized (Theorem~\ref{theo:equivalence} and Proposition~\ref{prop:determinization}, respectively). Unfortunately, these steps yield an automaton whose size is double exponential in the size of the original $\VA$. Therefore we look for more efficient translations. A first positive result is that, in the general case, we are able to transform a $\VA$ into a $\dsEVA$ avoiding the double exponential blowup.


\begin{proposition}\label{prop:general-VA}
	For any $\VA$ $\cA$ there exists an equivalent $\dsEVA$ $\cA'$ with at most $2^n3^\ell$ states and $2^n3^\ell(2^\ell+|\Sigma|)$ transitions.
\end{proposition}

As we can see, transforming an arbitrary $\VA$ results in a $\dsEVA$ that is exponential both in the number of states and in the number of variables of the original~$\VA$. Now, since it is common in practice to use the syntactic restrictions over RGX formulas that restrict VA to functional or sequential, we study whether we can do our translation more efficiently in these cases. It turns out that we can indeed avoid the exponential blowup in the number of variables in the functional case.

\begin{proposition}\label{prop:func-extended-blowup}
	For any functional $\VA$ $\cA$ there exists an equivalent $\dsEVA$ $\cA'$ with at most $2^n$ states and $2^n(n^2+|\Sigma|)$ transitions.
\end{proposition}

Unfortunately, for sequential $\VA$, we are not able to obtain a
similar reduction in the blowup in the number of variables. The reason
is that there is a blowup in the number of transitions when
transforming a sequential $\VA$ into an extended sequential $\VA$. To
illustrate, consider the automaton in
Figure~\ref{fig:badsequential}. Note that there, any path between $q_0$ and $q_F$ opens and closes exactly one
variable in $\{x_i,y_i\}$, for each $i\in\{1,\ldots,n\}$. Therefore,
to simulate this behavior in an extended \VA\ (which disallows two
consecutive variable transitions), we need $2^n$ transitions between
the initial and final states, one for each possible set of variables.

 \begin{figure}
 	\begin{center}
 		\resizebox{\columnwidth}{!}{
 			\begin{tikzpicture}[->,>=stealth',auto, thick, scale = 1.0,initial text= {}]
			
 			% The graph
 			\node [state,initial] at (0,0) (q0) {$q_0$};
 			\node [state] at (1.5,1) (q01) {};
 			\node [state] at (1.5,-1) (q02) {};		  
 			\node [state] at (3,0) (q1) {};
 			\node [state] at (4.5,1) (q11) {};
 			\node [state] at (4.5,-1) (q12) {};
 			\node [inner sep=2mm] at (6,0) (q2) {$\ldots$};
 			\node [state] at (7.5,1) (qn1) {};
 			\node [state] at (7.5,-1) (qn2) {};
 			\node [state] at (9,0) (qn) {$q$};
 			\node [state,accepting] at (11,0) (qf) {};
			
			
 			%\node [state,accepting] at (10,0) (q5) {$q_5$};
			
 			% Graph edges
 			\path[->] (q0) edge node[above] {$\Open{x_1} \ \ \ $} (q01);
 			\path[->] (q0) edge node[below] {$\Open{y_1} \ \ \ $} (q02);
 			\path[->] (q01) edge node[above] {$\ \ \Close{x_1}$} (q1);
 			\path[->] (q02) edge node[below] {$\ \ \Close{y_1}$} (q1);	  
 			\path[->] (q1) edge node[above] {$\Open{x_2} \ \ \ $} (q11);
 			\path[->] (q1) edge node[below] {$\Open{y_2} \ \ \ $} (q12);
 			\path[->] (q11) edge node[above] {$\ \  \Close{x_2}$} (q2);
 			\path[->] (q12) edge node[below] {$ \ \ \Close{y_2}$} (q2);
 			\path[->] (q2) edge node[above] {$\Open{x_n} \ \ \ $} (qn1);
 			\path[->] (q2) edge node[below] {$\Open{y_n} \ \ \ $} (qn2);
 			\path[->] (qn1) edge node[above] {$\ \ \Close{x_n}$} (qn);
 			\path[->] (qn2) edge node[below] {$\ \ \Close{y_n}$} (qn);
 			\path[->] (qn) edge node[above] {$a$} (qf);
 			\end{tikzpicture}
 		}
 	\end{center}
 	\vspace*{-15pt}
 	\caption{A sequential VA with $l$ variables such that every equivalent  extended VA has $O(2^l)$ transitions.}
 	\label{fig:badsequential}
 \end{figure}

\begin{proposition}\label{prop:seq-extended-existance}
	For every $k>0$ there is a sequential VA $\cA$ with $3k+2$ states and $4k+1$ transitions, such that for every extended VA $\cA'$ equivalent to $\cA$ it is the case that $\cA'$ has at least $2^k$ transitions.
\end{proposition}

As illustrated by our example, this exponential blowup originates from mappings that contain empty spans, i.e. variables that are closed immediately after they are open. We say that a VA $\cA$ is $\epsilon$-free if for every document $d$ and mapping $\mu\in\semd{\cA}$, $\mu$ does not define a span of the form $[i,i\rangle$, for $i\in\mathbb{N}$. We show that the exponential blowup disappears for $\epsilon$-free sequential $\VA$.

\begin{proposition}\label{prop:seq-extended-blowup}
	For any sequential $\VA$ $\cA$ there exists an equivalent $\dsEVA$ $\cA'$ with at most $2^n$ states and $2^n(2^\ell n^2+|\Sigma|)$ transitions. Moreover, if $\cA$ is $\epsilon$-free $\cA'$ has $2^n(n^2+|\Sigma|)$ transitions.
\end{proposition}

It is important to note that the previous results are relevant for evaluating regular spanners because any RGX formula can be converted into a VA in linear time~\cite{FKRV15} and, furthermore, if the RGX formula is sequential (resp. functional), then the resulting VA will also be sequential~\cite{MaturanaRV17} (resp. functional~\cite{FKRV15}). 

Now that we understand how to transform a $\VA$ into a $\dsEVA$, we
proceed to study how to apply the algebraic operators to evaluate
regular spanners.  In~\cite{FKRV15}, it was shown that any regular
spanner is in fact equivalent to a VA showing effective
constructions. In particular, it is known that for every pair of VA
$\cA_1$ and $\cA_2$, there exists a VA $\cA$ of exponential size such
that $\semd{\cA} = \semd{\cA_1} \bowtie \semd{\cA_2}$. The exponential
blowup comes from the fact that each transition is equipped at most
with one variable and two variable transitions can occur
consecutively. Therefore, one needs to consider all possible orders of
consecutive variable transitions when computing a product (see
\cite{FaginKRV15}). However, if the automata are functional it is
known that we can avoid this blowup~\cite{FreydenbergerKP17}, and that
in this case $\cA$ has quartic size $O(l n^4)$. Because we allow for
multiple variable operations in a single transition in extended $\VA$,
this quartic size becomes quadratic for extended VA.

\begin{proposition}\label{prop:join-regular-spanners}
	For any pair of $\EVA$ $\cA_1$ and $\cA_2$, there exists an $\EVA$ $\cA'$ of quadratic size such that $\cA'\equiv\cA_1 \Join \cA_2$. Moreover, if $\cA_1$ and $\cA_2$ are both functional or deterministic, then $\cA'$ is also functional or deterministic, respectively.
\end{proposition}

Unfortunately, if $\cA_1$ and $\cA_2$ are sequential, then the resulting automaton $\cA'\equiv\cA_1 \Join \cA_2$ is not necessarily sequential. The problem lies in the fact that, to construct a sequential product, we would need to keep track of which variables have been processed by which automaton. This can be avoided for functional automata as we know that both automata have to open and close all variables at the same time.

Now we proceed to study union. Again, we obtain that for sequential automata this can be done efficiently without losing sequentiality or determinism.

\begin{proposition}\label{prop:union-regular-spanners}
	For any pair of $\EVA$ $\cA_1$ and $\cA_2$, there exists an $\EVA$ $\cA''$ of quadratic size such that $\cA''\equiv\cA_1 \cup \cA_2$. Moreover, if $\cA_1$ and $\cA_2$ are both sequential or deterministic, then $\cA''$ is also sequential or deterministic, respectively.
\end{proposition}

The quadratic size is required because, to preserve determinism, one needs to construct the union by means of a modified product. This construction works also for functional $\EVA$, given that functional $\EVA$ is a special case of sequential $\EVA$.

Following the previous results, we can transform a functional $\VA^\algnoproj$ expression into a single $\dsEVA$ with a single exponential blowup: first, we transform each functional $\VA$ into a $\dsEVA$, and then compute the corresponding unions and joins.

\begin{proposition}\label{prop:expressions-to-va}
	Consider a $\VA^\algnoproj$ expression mentioning functional VAs $\cA_1,\ldots,\cA_k$. Let $n_i$, $m_i$ and $\ell_i$ be the number of states, transitions and variables of $\cA_i$, respectively. Then, there exists an equivalent $\dsEVA$ with at most $2^{\sum_i n_i}$ states and $2^{\sum_i n_i}\cdot(\sum_i n_i^2 + |\Sigma|)$ transitions.
\end{proposition}

The reason why we need to use a $\VA^\algnoproj$ expression instead of a $\VA^\algops$ expression is because projection does not preserve determinism in the automaton, and therefore we need to determinize the automaton at the end, producing a double exponential blowup. Also, if we start from a sequential $\VA^\algops$ expression we will incur in a double exponential blowup, even if we disallow projections. 
Therefore, by combining the previous propositions for the case of $\VA^\algnoproj$ expressions over sequential $\VA$ or, more general, for  $\VA^\algops$ expressions over functional $\VA$ we can build a $\dsEVA$ of double exponential size. 
We leave as an open problem how to build a $\dsEVA$ of single exponential size from a  $\VA^\algops$ expression.

%Surprisingly (and as a very positive result) we show that we can achieve a double exponential blowup in the general case; even for non-sequential $\VA^\algops$ expressions.
%\begin{proposition}
%	Consider a $\VA^\algops$ expression mentioning VAs $\cA_1,\ldots,\cA_k$. Let $n_i$, $m_i$ and $\ell_i$ be the number of states, transitions and variables of $\cA_i$, respectively. Then, there is an equivalent SDEVA with at most $XXX$ states, $XXXX$ transitions and $\sum_{i=1}^k\ell_i$ variables.
%\end{proposition}

Having these results, we can finally show the precise time required by our algorithm in order to evaluate expressions.

\begin{corollary}
	Consider a document $d$ and a $\VA^\algnoproj$ expression $\gamma$ mentioning functional VAs $\cA_1,\ldots,\cA_k$. Let $n_i$, $m_i$ and $\ell_i$ be the number of states, transitions and variables of $\cA_i$, respectively.
	Then, $\semd{\gamma}$ can be enumerated with constant delay after a preprocessing phase of time $O(2^{\sum_i n_i}(\sum_i n_i^2 + |\Sigma|))$.
\end{corollary}

% When the expression is functional, we have a double exponential blowup. We first need to transform each sequential automaton into its extended version, then compute the joins and unions, and determinize the result. To do this, we use the following proposition.

% \begin{proposition}\label{prop:single-regular-spanners}
% 	Let $\cA_1$ and $\cA_2$ be extended VA. There exist extended $\VA$ $\cA'$ and $\cA''$ of quadratic size such that $\cA'\equiv\cA_1 \Join \cA_2$ and $\cA''\equiv\cA_1 \cup \cA_2$.
% \end{proposition}

% Unfortunately, as already shown in Proposition~\ref{prop:seq-extended-blowup} transforming a sequential $\VA$ into an extended $\VA$ is already exponential. This yields a double exponential blowup:

% \begin{proposition}
% 	Consider a $\VA^\algnoproj$ expression mentioning VAs $\cA_1,\ldots,\cA_k$. Let $n_i$, $m_i$ and $\ell_i$ be the number of states, transitions and variables of $\cA_i$, respectively. Then, there is an equivalent SDEVA with at most $XXX$ states, $XXXX$ transitions and $\sum_{i=1}^k\ell_i$ variables.
% \end{proposition}



% \begin{proposition}
% 	Consider a $\VA^\algnoproj$ expression mentioning VAs $\cA_1,\ldots,\cA_k$. Let $n_i$, $m_i$ and $\ell_i$ be the number of states, transitions and variables of $\cA_i$, respectively. Then, there is an equivalent $\dsEVA$ with at most $XXX$ states, $XXXX$ transitions and $\sum_{i=1}^k\ell_i$ variables.
% \end{proposition}






% \begin{proposition}
% 	Consider a $\VA^\algops$ expression mentioning VAs $\cA_1,\ldots,\cA_k$. Let $n_i$, $m_i$ and $\ell_i$ be the number of states, transitions and variables of $\cA_i$, respectively. Then, there is an equivalent SDEVA with at most $XXX$ states, $XXXX$ transitions and $\sum_{i=1}^k\ell_i$ variables.
% \end{proposition}

% Surprisingly, one of the two exponential blowups originates from projections. The reason behind this is that, in order to avoid an additional exponential blowup we convert the automata to SDEVA before applying the join operations. This allows us to avoid one exponential blowup, in particular because the product of extended VA can be done in quadratic time (see Appendix~XXX). The problem with projection is that it can turn a deterministic VA into a non-deterministic one. The result then needs to be determinized again, resulting in a double blowup. This step can be avoided if the original expression does not contain projection.

% \begin{proposition}
% 	Consider a $\VA^\algnoproj$ expression mentioning VAs $\cA_1,\ldots,\cA_k$. Let $n_i$, $m_i$ and $\ell_i$ be the number of states, transitions and variables of $\cA_i$, respectively. Then, there is an equivalent SDEVA with at most $XXX$ states, $XXXX$ transitions and $\sum_{i=1}^k\ell_i$ variables.
% \end{proposition}

% As we can see, transforming an arbitrary $\VA^\algnoproj$ results in a SDEVA that is exponential both in the number of states and in the number of variables of the original VA. Now, since it is common in practice to use the syntactic restrictions over RGX formulas that restrict VA to functional or sequential, we study whether we can do our translation more efficiently in these cases. It turns out that we can indeed avoid the exponential blowup in the number of variables in the functional case.

% \begin{proposition}
% 	Consider a $\VA^\algnoproj$ expression mentioning VAs $\cA_1,\ldots,\cA_k$, which are all functional. Let $n_i$, $m_i$ and $\ell_i$ be the number of states, transitions and variables of $\cA_i$, respectively. Then, there is an equivalent SDEVA with at most $XXX$ states, $XXXX$ transitions and $\sum_{i=1}^k\ell_i$ variables.
% \end{proposition}

% Unfortunately, for the case of sequential automata the blowup in the number of variables cannot be avoided. The reason behind this is that it is not possible to translate in polynomial time a sequential VA into an extended sequential VA. We give some intuition behind this blowup in Figure~\ref{fig:badsequential}. Note that in the automaton of this figure, any path between $q_0$ and $q_F$ opens and closes exactly one variable in $\{x_i,y_i\}$, for each $i\in\{1,\ldots,n\}$. Therefore, to simulate this behavior in an extended VA (which disallows two consecutive variable transitions), we need $2^n$ transition between the initial and final states, one for each possible set of variables.

% \begin{proposition}\label{prop:seq-extended-blowup}
% 	For every $k>0$ there is a sequential VA $\cA$ with $3k+3$ states and $4k+1$ transitions, such that for every extended VA $\cA'$ such that $\cA\equiv\cA'$ it is the case that $\cA'$ has at least $2^k$ transitions.
% \end{proposition}

% As illustrated by Figure~\ref{fig:badsequential}, this exponential blowup originates from mappings that contain $\varepsilon$-spans, i.e. variables that are closed immediately after they are open. If this is not the case, then the exponential blowup disappears. We say that a VA $\cA$ is $\epsilon$-free if for every document $d$ and mapping $\mu\in\semp{\cA}{d}$, $\mu$ does not define a span of the form $[i,i\rangle$, for $i\in\mathbb{N}$.

% \begin{proposition}
% 	Consider a $\VA^\algnoproj$ expression mentioning VAs $\cA_1,\ldots,\cA_k$, which are all sequential and $\epsilon$-free. Let $n_i$, $m_i$ and $\ell_i$ be the number of states, transitions and variables of $\cA_i$, respectively. Then, there is an equivalent SDEVA with at most $XXX$ states, $XXXX$ transitions and $\sum_{i=1}^k\ell_i$ variables.
% \end{proposition}

% Therefore, if a sequential VA does not produce mappings with empty spans, we can also avoid the blowup in the number of variables.

% Having all these results we can finally state what is the exact complexity of the evaluating a $\VA^\algops$ with the expression algorithm presented in Section~\ref{sec:algorithm}, depending on the form of the automata in the expression.

% \begin{proposition}
% 	Let $d$ be a document and let $\gamma$ be an expression in $\VA^\algnoproj$, mentioning VAs $\cA_1,\ldots,\cA_k$. Algorithm~\ref{alg:ma-eval} enumerates $\semp{\gamma}{d}$ with constant delay after a preprocessing phase of time $O(XXX)$. Moreover, if every automaton in $\cA_1,\ldots,\cA_k$ is either functional or sequential and $epsilon$-free, then the preprocessing phase takes time $O(XXX)$
% \end{proposition}

% This result gives us a good understanding of the practical efficiency with which we can evaluate regular spanners. Unfortunately, if we include projection the preprocessing phase implies an extra exponential blowup.



% %####################################
% %####################################
% %####################################
% %####################################


% Given that any regular spanner is equivalent to a VA~\cite{FKRV15} and that any VA is equivalent to a sequential deterministic extended VA (by Theorem~\ref{theo:equivalence} and Proposition~\ref{prop:determinization}), this implies that a regular spanner can be evaluated with constant delay enumeration after $O(|f(\cA)| \times |d|)$ preprocessing time, where $f(\cA)$ is the function that converts a regular spanner into an equivalent sequential deterministic extended VA.

% \martin{Here we should shortly mention previous work (the non-elementary preprocessing), so the results sound stronger.}

% In this section, we present a fine-grained study of the complexity of transforming an arbitrary regular spanner to a sequential deterministic extended VA, putting in perspective what is the cost of using the algorithm of Section~\ref{sec:algorithm} for evaluating regular spanners. Since RGX formulas can be translated into VA in linear time~\cite{FKRV15}, we consider expressions in $\VA^\algops$.

% If we inspect the different constructions presented, starting from an expression in $\VA^\algops$ we can first convert it into a single VA. This VA can then be converted into a sequential VA by using a construction similar to that presented in \cite{F17}. Finally, this sequential VA can be extended and determinized (Theorem~\ref{theo:equivalence} and Proposition~\ref{prop:determinization}, respectively). Finally we can run our algorithm
%  By Theorem~\ref{theo:equivalence}, this VA can be turned into an extended VA which can be then transformed into its deterministic, extended and sequential version (Theorem~\ref{theo:equivalence}). Then to finally apply the algebraic operators. However, if we follow each one of the translations in a sequence, we end up with an automaton that is double exponential in the size of the regular spanner. Fortunately, in some cases this translation can be done more efficiently if some steps are combined together in a single transformation. In particular, since RGX formulas can be translated into VA in linear time, we start from an expression in 



% %We discuss first the case of general VA, to then discuss the case of spanner algebras.

% %As discussed in the previous section, in terms of data complexity this evaluation can be done in linear time in the size of the input string. However, to achieve this complexity we need a deterministic extended vset automaton that is equivalent to the original spanner algebra expression. In this section we present a fine-grained study of the complexity of transforming an arbitrary spanner algebra expression into a deterministic extended vset automaton.\par


% Regular spanners are defined by combining RGX formulas with projections, unions, and joins. In~\cite{FKRV15}, it was shown that any regular spanner is in fact equivalent to a VA showing effective constructions. In particular, it is known that any RGX formula can be converted into a VA in linear time~\cite{FKRV15} and, furthermore, if the RGX formula is sequential (resp. functional), then the resulting VA will also be sequential~\cite{MaturanaRV17} (resp. functional~\cite{FKRV15}). Moreover, for every pair of VA automata $\cA_1$ and $\cA_2$, there exists a VA $\cA$ of exponential size such that $\semd{\cA} = \semd{\cA_1} \bowtie \semd{\cA_2}$. The exponential blowup comes from the fact that each transition is equipped at most with one variable and two variable transitions can occur consecutively. Therefore, one needs to consider all possible orders of consecutive variable transitions when computing a product (see \cite{FaginKRV15}). However, if we allow for multiple variable operations in a single transition, we can avoid this blowup. This is the main motivation for using extended VA.

% \begin{proposition}\label{prop:single-regular-spanners}
% 	Let $\cA_1$ and $\cA_2$ be extended VA and let $X$ be a set of variables. There exist extended VA of at most linear size equivalent to $\pi_{X} \cA_1$ and $\cA_1 \cup \cA_2$. Furthermore, there exists an extended VA of quadratic size that is equivalent to $\cA_1 \bowtie \cA_2$.
% \end{proposition} 

% Note that avoiding this blowup does not prevent us from an exponential result when transforming an arbitrary expression to an extended VA, as the result can be exponential in the number of joins in the expression.

% To take advantage of the previous result and the evaluation algorithm, we also need to transform arbitrary VA into their sequential extended version. We start by transforming VA into their sequential version, to then extend them with sets of variables. Freydenberger \cite{F17} proved that any VA with $n$ states and $\ell$ variables can be transformed into an equivalent functional VA with $n\cdot 3^\ell$ states. We show that this is also the case if we want to construct a sequential VA.
% \begin{proposition}
% 	Given a VA with $n$ states and $\ell$ variables, there is an equivalent sequential VA with $n\cdot 3^\ell$ states.
% \end{proposition}
% \martin{Need to check this.}

% Now we need to compute the extended version of sequential VA. Unfortunately, there is an exponential blowup in this conversion.

% % \begin{proposition}\label{prop:seq-extended-blowup}
% % 	Let $\cA$ be a functional (sequential) VA with $n$ states, $m$ transitions and $\ell$ variables. There is an equivalent functional (resp. sequential) extended VA with at most $n$ states and $O(m+n^2)$ transitions (resp. $O(m + 2^\ell \cdot n^2)$ transitions).
% % \end{proposition}

% \begin{proposition}\label{prop:seq-extended-blowup}
% 	Let $\cA$ be a sequential VA with $n$ states, $m$ transitions and $\ell$ variables. There is an equivalent sequential extended VA with at most $n$ states and $O(m + 2^\ell \cdot n^2)$.
% \end{proposition}

% Next we show that this exponential blowup is unavoidable. To illustrate this, consider the VA depicted in Figure~\ref{fig:badsequential}. Any path between $q_0$ and $q_F$ opens and closes exactly one variable in $\{x_i,y_i\}$, for each $i\in\{1,\ldots,n\}$. Therefore, to simulate this behavior in an extended VA (disallowing two sequential variable transitions), we need $2^n$ transition between $q_0$ and $q_F$, one for each possible set of variables.

% \begin{proposition}\label{prop:seq-extended-blowup}
% 	For every $k>0$ there is a sequential VA $\cA$ with $3k+3$ states and $4k+1$ transitions, such that for every extended VA $\cA'$ such that $\cA\equiv\cA'$ it is the case that $\cA'$ has at least $2^k$ transitions.
% \end{proposition}

% However, this exponential blowup originates only from mappings that contain $\varepsilon$-spans, i.e. variables that are closed immediately after they are open. If this is not the case, then the exponential blowup disappears. We say that a VA $\cA$ is $\epsilon$-free if for every document $d$ and mapping $\mu\in\semp{\cA}{d}$, $\mu$ does not define a span of the form $[i,i\rangle$, for $i\in\mathbb{N}$.

% \begin{proposition}
% 	Given an $\epsilon$-free sequential VA $\cA$ with $n$ states and $m$ transitions, one can construct an equivalent sequential extended VA with at most $n$ states and $O(m + n^2)$ transitions, in time $O(m+n^2)$.
% \end{proposition}

% The algorithm presented in Section~\ref{sec:algorithm} not only requires a sequential VA, but also a deterministic one. Therefore we also study the problem of determinizing sequential VA.

% \begin{proposition}
% 	Given an $\epsilon$-free sequential VA $\cA$ with $n$ states and $m$ transitions, one can construct an equivalent sequential extended VA with at most $n$ states and $O(m + n^2)$ transitions, in time $O(m+n^2)$.
% \end{proposition}

% To solve the blowup in general, it seems resonable to introduce a \emph{symbolic} representations for sets of variables. Unfortunately, if this is done in the natural way the enumeration procedure presented in Section~\ref{sec:algorithm} does not provide constant delay. We leave a general study of whether sequential VA can be transformed into extended sequential VA in polynomial time for future work.









% \subsection{CDE for variable set automata}\label{ss:rgx}

% We know that any RGX formula can be converted into a VA in linear time~\cite{FKRV15} and, furthermore, if the RGX formula is sequential (resp. functional), then the resulting VA will also be sequential~\cite{MaturanaRV17} (resp. functional~\cite{FKRV15}). Since the algorithm presented in 

% As it was shown in~\cite{MaturanaRV17}, sequential VA have good algorithmic properties and, furthermore, can be evaluated with polynomial delay in terms of combined complexity. \martin{Cristian, please give the exact bounds.} To derive an algorithm for this class, we first need to convert a sequential VA into its extended version, to then apply its determinization. 
% One can easily show that converting any VA into an equivalent extended VA takes exponential time in the worst case. Interestingly, this construction can be done in polynomial time for functional VA.

% In order to evaluate a regular spanner, we transform it to an algebraic expression using VA. As the algorithm presented in Section~\ref{sec:algorithm} requires a deterministic sequential VA, we start by studying how to we will transform the regular spanner into an algebraic expression between VA.

% \stijn{TO DISCUSS: Freydenberger, in his ICDT 2017 paper, has some results about the blow-up from normal automata to functional automata. (see proposition 12)Is this relevant in our context?}

% \begin{proposition}
% 	Given a functional VA $\cA$ with $n$ states and $m$ transitions, one can construct an equivalent functional extended VA with at most $n$ states and $O(m + n^2)$ transitions, in time $O(m+n^2)$.
% \end{proposition}


% Unfortunately, to go from sequential VA into its extended version one
% has an exponential blowup in the number of variables that is
% unavoidable in some cases.  
% \stijn{At current, the proposition only mentions that it can be done
%   in this size, but not that this is unavoidable. I would add  to the
%   following proposition also the statement that it is unavoidable,
%   i.e., there exist sequantial VA for which any equivalent sequential
%   extended VA has $2^\ell$ states.}
% \begin{proposition}\label{prop:seq-extended-blowup}
% 	Given a sequential VA $\cA$ with $n$ states, $m$ transitions and $\ell$ variables, one can construct an equivalent sequential extended VA with at most $n$ states and $O(m + 2^\ell \cdot n^2)$ transitions.
% \end{proposition}
% \begin{figure}
% 	\begin{center}
% 		\resizebox{\columnwidth}{!}{
% 			\begin{tikzpicture}[->,>=stealth',auto, thick, scale = 1.0,initial text= {}]
			
% 			% The graph
% 			\node [state,initial] at (0,0) (q0) {$q_0$};
% 			\node [state] at (1.5,1) (q01) {};
% 			\node [state] at (1.5,-1) (q02) {};		  
% 			\node [state] at (3,0) (q1) {};
% 			\node [state] at (4.5,1) (q11) {};
% 			\node [state] at (4.5,-1) (q12) {};
% 			\node [inner sep=2mm] at (6,0) (q2) {$\ldots$};
% 			\node [state] at (7.5,1) (qn1) {};
% 			\node [state] at (7.5,-1) (qn2) {};
% 			\node [state] at (9,0) (qn) {$q$};
% 			\node [state,accepting] at (11,0) (qf) {};
			
			
% 			%\node [state,accepting] at (10,0) (q5) {$q_5$};
			
% 			% Graph edges
% 			\path[->] (q0) edge node[above] {$\Open{x_1} \ \ \ $} (q01);
% 			\path[->] (q0) edge node[below] {$\Open{y_1} \ \ \ $} (q02);
% 			\path[->] (q01) edge node[above] {$\ \ \Close{x_1}$} (q1);
% 			\path[->] (q02) edge node[below] {$\ \ \Close{y_1}$} (q1);	  
% 			\path[->] (q1) edge node[above] {$\Open{x_2} \ \ \ $} (q11);
% 			\path[->] (q1) edge node[below] {$\Open{y_2} \ \ \ $} (q12);
% 			\path[->] (q11) edge node[above] {$\ \  \Close{x_2}$} (q2);
% 			\path[->] (q12) edge node[below] {$ \ \ \Close{y_2}$} (q2);
% 			\path[->] (q2) edge node[above] {$\Open{x_n} \ \ \ $} (qn1);
% 			\path[->] (q2) edge node[below] {$\Open{y_n} \ \ \ $} (qn2);
% 			\path[->] (qn1) edge node[above] {$\ \ \Close{x_n}$} (qn);
% 			\path[->] (qn2) edge node[below] {$\ \ \Close{y_n}$} (qn);
% 			\path[->] (qn) edge node[above] {$a$} (qf);
% 			\end{tikzpicture}
% 		}
% 	\end{center}
% 	\vspace*{-15pt}
% 	\caption{A sequential VA with $l$ variables such that every equivalent  extended VA has $O(2^l)$ transitions.}
% 	\label{fig:badsequential}
% \end{figure}
% \martin{Do we have any result regarding the exponential blowup? If not, I'll have a small discussion stating that we don't know but this is the intuition. As the presentation is now there is not much intuition because the reader will not be familiar with the construction. Moreover it sounds rather strange}
% To understand why there is an exponential blow-up on the number of transition, consider the sequential VA of Figure~\ref{fig:badsequential}. These automaton has $2n$ variables and to transform it into an extended automaton one needs to add all set transitions of the form $(q_0, \bigcup_{i\in P} \{\Open{x_i}, \Close{x_i}\} \cup \bigcup_{i \in P^c} \{\Open{y_i}, \Close{y_i}\},  q)$ for every $P \subseteq \{1, \ldots, 2n\}$ and $P^c = \{1, \ldots, 2n\} -P$.

% The example in Figure~\ref{fig:badsequential} illustrates that the source of this exponential blow-up is rooted in the possibility of output mappings with $\epsilon$-spans, namely, a mapping $\mu$ such that $\mu(x) = [i,i\rangle$ for some $x$ and $i$.
% One can argue that these mappings are not useful in some practical scenarios given that they extract no content of the document and, furthermore, they can be easily removed from the output of a mapping.
% This motivates the following definitions and result. We say that a VA $\cA$ is $\epsilon$-free if for every document $d$, no $\mu \in \sem{\cA}_d$ has $\epsilon$-spans. 
% \begin{proposition}
% 	Given an $\epsilon$-free sequential VA $\cA$ with $n$ states and $m$ transitions, one can construct an equivalent sequential extended VA with at most $n$ states and $O(m + n^2)$ transitions, in time $O(m+n^2)$.
% \end{proposition}

% Therefore, if a sequential VA does not require to output mappings with $\epsilon$-spans, we can avoid the blowup of Proposition~\ref{prop:seq-extended-blowup} by having quadratic reductions to extended VA, similar to the functional case.

% Now, in order to apply the algorithm of Section~\ref{sec:algorithm} we need to transform our sequential or functional VA into a deterministic extended VA. By combining the previous results and the the algorithm of Section~\ref{sec:algorithm}, we get a constant delay algorithm that has an exponential blowup in the number of states.
% \begin{corollary}\label{cor:determinization-cost}
% 	Let $d$ be a document and let $\cA$ be a functional or $\epsilon$-free sequential VA with $n$ states and $m$ transitions. There is an algorithm that enumerates $\semd{\cA}$ with constant delay after a precomputation phase of $O(2^n \cdot (m + n^2) \cdot |d|)$.
% \end{corollary}

% It is worth mentioning that the exponential factor $2^n$ is not always necessary and depends on the ``interaction'' of the VA with the input. In practice, the evaluation can be done on-the-fly~\cite{XXX} accessing only the states of the determinization that are needed in each transition.

% In~\cite{F17}, it was shown that the decision version of evaluating any VA over a document (i.e. combined complexity) is $\NP$-complete. 
% Furthermore, this problem is FPT in the number of variables~\cite{MaturanaRV17} \martin{cite Benny's paper to appear in PODS 2018}. 
% Therefore, it comes at no surprise that the enumeration problem regarding any VA must have an additional blow-up in the number of variables if the mappings are output with constant-delay.
% \begin{proposition}
% 	Given any VA with $n$ states, $m$ transitions and $\ell$ variables, one can construct an equivalent sequential extended VA with at most $2^n \cdot (2\ell)!$ states and $O(2^n \cdot (2\ell)! \cdot (2^\ell + m))$ transitions.
% \end{proposition}

% A natural question at this point is whether we are forced to pay the exponential blow-up of Proposition~\ref{prop:seq-extended-blowup} or Corollary~\ref{cor:determinization-cost} for enumerating with constant-delay all outputs of a sequential VA over a document. 
% In Section~\ref{sec:lower}, we give our preliminaries results for answering this question, showing that the exponential cost appears unavoidable in a similar setting for counting the number of resulting mappings.

% \subsection{Spanner algebras}\label{ss:algebra}

% \martin{Add discussion about the exponential blowup of the join when the automaton is not extended. Note that this is the case even when constructing the product between functional VA.}
% Regular spanners are defined by combining RGX formulas with projections, unions, and joins. 
% In~\cite{FKRV15}, it was shown that any regular spanner is in fact equivalent to a VA showing effective constructions. 
% In particular, it was shown that for every pair of VA automata $\cA_1$ and $\cA_2$, there exists a VA $\cA$ of size exponential such that $\semd{\cA} = \semd{\cA_1} \bowtie \semd{\cA_2}$.
% In the next result we show that, if the operation of projection, union, and join are done through extended VA instead of VA, the constructions are much simpler taking at most quadratic time and space in the size of $\cA_1$ and $\cA_2$.

% \begin{proposition}\label{prop:single-regular-spanners}
% 	For every pair of extended VA $\cA_1$ and $\cA_2$, there exists extended VA of at most linear size for $\pi_{X} \cA_1$ and $\cA_1 \cup \cA_2$. Furthermore, there exists an extended VA of quadratic size for $\cA_1 \bowtie \cA_2$.
% \end{proposition} 

% The above VA construction are design for a single relational operation and can be used to apply the constant-delay algorithm of Section~\ref{sec:algorithm}.
% Unfortunately, if several joins are applied over $n$ RGX formulas, the construction in Proposition~\ref{prop:single-regular-spanners} implies an additional exponential blow-up without considering yet the exponential blow-up of determinizing the resulting VA.
% In fact, we show next that this apparently double exponential blow-up can be avoided by first determinizing the VA coming from RGX formulas to then apply the constructions from Proposition~\ref{prop:single-regular-spanners}.

% \begin{proposition}\label{prop:regular-spanners}
% 	Given a spanner expression with $n$ functional or $\epsilon$-free extended VA $\cA_1, \ldots, \cA_k$, each of them with $n_i$ states and $m_i$ transitions, one can construct an equivalent deterministic sequential extended VA with at most $2^{\sum_i n_i}$ states and $O(2^{\sum_i n_i} \cdot \sum_i (m_i+n_i^2))$ transitions.
% \end{proposition}

% \martin{Take out projection and discuss}

% It is worth noting that $\sum_i n_i$ is proportional to the total size of the spanner expression. Therefore, by applying the construction of Proposition~\ref{prop:regular-spanners} and the algorithm of Section~\ref{sec:algorithm} we get a constant-delay algorithm with precomputation phase of exponential time in the size of the expression, similar to Corollary~\ref{cor:determinization-cost}.
% In other words, relational operators over functional or  $\epsilon$-free sequential RGX do not increase the worst-case precomputation phase.



% %\cristian{Aqui va la versión antigua}
% %
% %%First, we need to note that a spanner algebra expression contains a set of ReGex formulas. We know by \cite{?} that each of these formulas can be translated into a functional VA in linear time. Then, each functional VA needs to be transformed into a functional EVA, for which we use the following result.
% %
% %\begin{proposition}
% %There is an algorithm that takes as input a functional VA $A$ and produces a functional EVA $A'$ such that $A\equiv A'$. Moreover, if $A$ has $n$ states and $m$ transitions then the algorithm runs in time $O(m+n^2)$, and the resulting automaton $A'$ has at most $n$ states and $O(m + n^2)$ transitions.
% %\end{proposition}
% %
% %Having a set of functional VA, we proceed to determinize each of them. As the following result shows, this process can be exponential in the number of states:
% %
% %\begin{proposition}
% %There is an algorithm that takes as input a functional EVA $A$ and produces a functional deterministic EVA $A'$ such that $A\equiv A'$. Moreover, if $A$ has $n$ states and $m$ transitions then the algorithm runs in time $O(2^n \cdot m \cdot |d|)$.
% %\end{proposition}
% %
% %Once we have translated each ReGeX formula into a functional and deterministic EVA, we need to compute the spanner operators, namely projections, unions and joins. We use the following proposition.
% %
% %\begin{proposition}
% %Let $\cA_1$ and $\cA_2$ be extended VA and let $X$ be a set of variables. There are extended vset automata $\cA^\pi_X$, $\cA_\cup$ and $\cA_\Join^X$, such that $\cA^\pi_X\equiv \pi_X\cA_1$, $\cA_\cup\equiv\cA_1\cup\cA_2$ and $\cA_\Join^X\equiv\cA_1 \bowtie_X \cA_2$. Furthermore, $\cA^\pi_X$ can be constructed in time $O(|\cA_1|)$, $\cA_\cup$ in time $O(|\cA_1|+|\cA_2|)$, and $\cA_\Join^X$ in time $O(|\cA_1|\cdot|\cA_2|)$.
% %\end{proposition}
% %
% %Once we have a deterministic functional EVA, we can run our constant-delay enumeration (in data complexity) algorithm. As the following Corollary shows, the preprocessing time, as well as the delay, can be exponential in the set of states of the automaton.
% %
% %\begin{corollary}
% %Let $d$ be a document and let $\cA$ be a deterministic functional VA with $n$ states and $m$ transitions. The algorithm presented in Section~\ref{sec:algorithm} enumerates the results $\cA(d)$ with delay $O(2^n \cdot (m + n^2))$, after a preprocessing stage that requires time
% %\[
% %O(2^n \cdot (m + n^2) \cdot |d|).
% %\]
% %\end{corollary}
% %
% %Finally, we have all the necessary ingredients to pinpoint the exact complexity of our processing-enumerating algorithm presented in the previous section.
% %
% %\begin{proposition}
% %	Let $d$ be a document, let $S$ be spanner expression with ReGeX formulas $r_1,\ldots,r_n$, and let $\cA_1, \ldots, \cA_n$ be the functional VA equivalent to $r_1,\ldots,r_n$, respectively. If for each $i\in\{1,\ldots,n\}$ the automaton $\cA_i$ has $n_i$ states and $m_i$ transitions, the algorithm presented in Section~\ref{sec:algorithm} can enumerate the results $S(d)$ with delay $O(2^{\sum_i n_i} \cdot \sum_i m_i)$ after a preprocessing time of
% %	\[
% %	O(2^{\sum_i n_i} \cdot \sum_i m_i \cdot |d|)
% %	\]
% %\end{proposition}
% %
% %\martin{the rest of this section is kept for comparison}
% %\subsection{Regex formulas and variable set automata}\label{ss:rgx}
% %
% %A first straightforward result is that determinizing a functional extended vset automaton requires an exponential blowup. Therefore, if our algorithm takes as input a functional extended vset automaton, the preprocessing phase will take time exponential in the size automaton.
% %
% %\begin{proposition}
% %There is an algorithm that takes as input a functional EVA $A$ and produces a functional DEVA $A'$ such that $A\equiv A'$. Moreover, if $A$ has $n$ states and $m$ transitions then the algorithm runs in time
% %\[O(2^n \cdot m \cdot |d|).\]
% %\end{proposition}
% %
% %We also require obtaining a functional EVA from a functional VA, which requires a quadratic step.
% %
% %\begin{proposition}
% %There is an algorithm that takes as input a functional VA $A$ and produces a functional EVA $A'$ such that $A\equiv A'$. Moreover, if $A$ has $n$ states and $m$ transitions then the algorithm runs in time $O(m+n^2)$. Moreover, the resulting automaton $A'$ has at most $n$ states and $O(m + n^2)$ transitions.
% %\end{proposition}
% %
% %\begin{proposition}
% %For any functional vset automaton with $n$-states and $m$-transitions there exists an equivalent functional extended vset automaton with $n$-states and at most $O(m+n^2)$ transitions.
% %\end{proposition}
% %
% %As a corollary of the previous two results we get the following.
% %
% %\begin{corollary}
% %For a functional vset automaton with $n$ states and $m$ transitions over a document $d$, the constant-delay algorithm takes preprocessing time of:
% %\[
% %O(2^n \cdot (m + n^2) \cdot |d|)
% %\]
% %\end{corollary}
% %
% %Here we can discuss that for functional RegEx formulas, the preprocessing time is the same. 
% %
% %Then we discuss the case of any vset automaton. In this case, one has the blowup of making the automata functional, extended, and deterministic. All of them can be done on-the-fly.
% %
% %\begin{proposition}
% %	For a vset automaton with $n$ states, $m$ transitions and $v$ variables over a document $d$, there exists a constant-delay algorithm that takes preprocessing time of:
% %	\[
% %	O(2^n \cdot (2v)! \cdot (2^v + m) \cdot |d|)
% %	\]
% %\end{proposition}
% %
% %
% %\subsection{Spanner algebras}\label{ss:algebra}
% %
% %In this section we study spanner algebra (i.e. projection, union, join) over functional extended vset automata. Given the results in the previous section, we know how to extend this results to functional or non-functional vset automata.
% %
% %First, we show that by using extended v-set automaton, the construction of projection, union and join takes polynomial time. 
% %
% %\begin{proposition}
% %For every pair of extended vset automata $\cA_1$ and $\cA_2$, there exists extended vset automata of at most linear size for $\pi_{X} \cA_1$ and $\cA_1 \cup \cA_2$. Furthermore, there exists an extended vset automaton of quadratic size for $\cA_1 \bowtie_X \cA_2$.
% %\end{proposition} 
% %
% %Here we should discuss that this construction is polynomial, compare to the construction given in the paper of Fagin et al.
% %
% %Now, we study how to extend the constant-delay algorithm for a spanner algebra expression over functional extended vset automata.
% %
% %\begin{proposition}
% %	For a spanner expression with functional extended vset automata $\cA_1, \ldots, \cA_n$ where each automaton $\cA_i$ has $n$ states and $m_i$ transitions and, there exists a constant-delay algorithm that takes preprocessing time of:
% %	\[
% %	O(2^{\sum_i n_i} \cdot \sum_i m_i \cdot |d|)
% %	\]
% %\end{proposition}


% %%% Local Variables: 
% %%% mode: latex
% %%% TeX-master: "../main/main"
% %%% End: 


==> union.tex <==

\subsubsection*{Join}
For any pair of $\fEVA$ $\cA_1$ and $\cA_2$, there exists an $\EVA$ $\cA'$ of quadratic size such that $\cA'\equiv\cA_1 \Join \cA_2$.

Let $\cA_1 = (Q_1, q_0^1, F_1, \delta_1)$ and $\cA_2 = (Q_2, q_0^2, F_2, \delta_2)$ be two $\fEVA$. Let $\VV_1 = \var(\cA_1)$, $\VV_2 = \var(\cA_2)$ and $\VV_\Join = \VV_1 \cap \VV_2$. The intuition behind the following construction is similar too the construction for intersection of NFAs: we run both automaton in parallel, adding the possibility to use at the same time markers from both automaton, but, only when both use the same markers from $\markers_{\VV_\Join}$.

Then, $\cA' = (Q_1 \times Q_2 , (q_0^1, q_0^2), F_1 \times F_2, \delta)$ where $\delta$ is defined as follows: 

\begin{itemize}
\item $\big( (p_1,p_2), a, (q_1. q_2))\big)\in\delta$ whenever $a \in \Sigma$, $(p_1,a,q_1) \in \delta_1$ and $(p_2,a,q_2) \in \delta_2$
\item $\forall p_2\in Q_2$, $\big( (p_1,p_2), S_1, (q_1, p_2))\big)\in\delta$ whenever $(p_1,S_1,q_1) \in \delta_1$ and $S_1\cap \markers_{\VV_\Join} = \emptyset$ 
\item $\forall p_1\in Q_1$, $\big( (p_1,p_2), S_2, (p_1, q_2))\big)\in\delta$ whenever $(p_2,S_2,q_2) \in \delta_2$ and $S_2\cap \markers_{\VV_\Join} = \emptyset$  
\item $\big( (p_1,p_2), S_1\cup S_2, (q_1, q_2))\big)\in\delta$ whenever $(p_1,S_1,q_1) \in \delta_1$ and $(p_2,S_2,q_2) \in \delta_2$ and 

$S_1 \cap \markers_{\VV_\Join} = S_2 \cap \markers_{\VV_\Join} $

\end{itemize}

To show that $\semd{\cA'} \subseteq \semd{\cA_1} \Join \semd{\cA_2}$, let $\mu$ be a  specific mapping in $\semd{\cA'}$ for the document $d$, and the corresponding valid and accepting run $\rho_\mu$ for $d$ that open and closes correctly all defined variables in $\mu$. From $\rho_\mu$, a sequence of states in $\cA_1$ and $\cA_2$ are established, that can define runs $\rho_1$ and $\rho_2$ in their respective automaton, thanks to the construction, using their respective existing transitions. This preserves both order of markers use and positions of use. Since $\cA_1$ and $\cA_2$ are functional, since $\rho_\mu$ is accepting, so are $\rho_1$ and $\rho_2$ and therefore are also valid, then $\mu^{\rho_1} \in \semd{\cA_1}$ and $\mu^{\rho_2} \in \semd{\cA_2}$. Finally, since all common marker transitions are performed by both automaton at the same union transitions, then $\mu^{\rho_1} \sim \mu^{\rho_2}$ and therefore $\mu = \mu^{\rho_1} \cup \mu^{\rho_2} \in \semd{\cA_1} \Join \semd{\cA_2} $. To show that $\semd{\cA_1} \Join \semd{\cA_2} \subseteq \semd{\cA'}$, let $\mu_1\in\semd{\cA_1}$, $\mu_2\in\semd{\cA_2}$ such that $\mu_1 \sim \mu_2$ and their corresponding runs be $\rho^{\mu_1}$ and $\rho^{\mu_2}$, respectively. Since they are compatible, then both runs use each marker in $\markers{\VV_\Join}$ in the same positions of $d$. Therefore, by merging the marker transitions made in each run, the corresponding union transitions must exists in $\cA'$ and used to construct a run $\rho$ in $\cA'$. Finally, since $\rho_1$ and $\rho_2$ are accepting, valid and total; the order is preserved and each variable appears once in $\rho$, then $\rho$ is also accepting, valid and total for $\var(\cA_1) \cup \var(\cA_2)$, then $\mu^{\rho} \in \semd{\cA'}$. It is easy to see that $\mu^{\rho} = \mu_1 \cup \mu_2$, and therefore $\mu_1 \cup \mu_2 \in \semd{\cA'}$.


To show that $\cA'$ is also functional, let $\rho$ be an accepting run in $\cA'$ for $d$. Thanks to the construction, and as shown before, corresponding runs in $\cA_1$ and $\cA_2$ can be produced from $\rho$ that are also accepting, and therefore valid and total since they are functional. Since all common markers are used in the same positions and once in the corresponding runs, so it does in $\rho$. Also, all variables are used in $\cA_1$ and $\cA_2$ runs, therefore is valid and total for $\var(\cA_1) \cup \var(\cA_2)$.

$\cA'$ has $|Q_1|\times |Q_2|$ states and at most $O(|\delta_1| \times |\delta_2|)$ because of the adding of union transitions. Therefore, is quadratic in size.
\subsubsection*{Projection}

Let $\cA$ be a $\fEVA$ and $Y\subset \VV$, there exists $\EVA$ $\cA_\pi$ such that $\cA_\pi \equiv \pi_Y \cA_1 $ of linear size.

To prove this, first we introduce the notion of $\epsilon$ transitions in $\EVA$, as the usual notion for regular NFA, namely, transition of the form $(q, \epsilon, p)$. If a run uses an $\epsilon$ transition, this produces no effect on the document read or variables that are open or close and are performed between regular letter transitions and extended marker transitions.

Let $\cA =(Q,q_0, F,\delta )$ be a $\fEVA$ and $Y\subset \VV$. Let $U = \markers_\VV \setminus \markers_Y$ be markers for unprojected variables, then $\cA' = (Q,q_0, F, \delta')$ where $\delta'$ is formed by $\delta$'s letter transitions $(q,a,p), a\in \Sigma$, and extended marker transitions without the unprojected variables but omiting the case that $\emptyset$ transitions are left, namely, $(q,S \setminus U,p)$ whenever $S\setminus U \neq \emptyset$ and $(q,\epsilon,p)$ when $S \setminus U = \emptyset$.

Equivalence is straightforward, for every $\mu \in \semd{\cA}$, exists a corresponding accepting and valid run $\rho$ in $\cA$, for which it exists a run $\rho'$ in $\cA'$ formed by the same sequence of states, but extended marker or $\epsilon$ transitions are used that only contain markers from $Y$. $\rho$ must also be valid since it maintains the order for $Y$ variables used in $\rho$.  This shows that $\pi_Y \semd{\cA} \subseteq \semd{\cA'}$.  $\semd{\cA'} \subseteq \pi_Y \semd{\cA}$ follows from the fact that $\cA'$ has no additional accepting paths in comparison to $\cA$. Is also easy to see that $\cA'$ must also be functional.

Note that, as for classical NFAs, from $\cA'$ an equivalent $\epsilon$ transition free $\EVA$ can constructed using $\epsilon$ closure over states. 

\subsubsection*{Union}

The following construction is the trivial disjointed state union of automaton with $\epsilon$ transitions to each corresponding initial state. Let $\cA_1 = (Q_1, q_0^1, F_1, \delta_1)$ and $\cA_2 = (Q_2, q_0^2, F_2, \delta_2)$ be two $\fEVA$ such $Q_1\cap Q_2 = \emptyset$. Then, let $\cA' = (Q_1\cup Q_2, q_0, F_1\cup F_2, \delta_1\cup \delta_2 \cup \{ (q_0, \epsilon, q_0^1), (q_0, \epsilon, q_0^2) \} )$. This simply adds an new initial state that connects to both automaton's initial states. Therefore every run in $\cA'$ must produce a run from $\cA_1\cup\cA_2$ and vice versa. An equivalent $\epsilon$ transition free automaton can be constructed as in the projection case. 

